Cross-Domain Latent Modulation for Variational Transfer Learning

We propose a cross-domain latent modulation mechanism within a variational autoencoders (VAE) framework to enable improved transfer learning. Our key idea is to procure deep representations from one data domain and use it as perturbation to the reparameterization of the latent variable in another domain. Specifically, deep representations of the source and target domains are first extracted by a unified inference model and aligned by employing gradient reversal. Second, the learned deep representations are cross-modulated to the latent encoding of the alternate domain. The consistency between the reconstruction from the modulated latent encoding and the generation using deep representation samples is then enforced in order to produce inter-class alignment in the latent space. We apply the proposed model to a number of transfer learning tasks including unsupervised domain adaptation and image-toimage translation. Experimental results show that our model gives competitive performance.

==> sections/appendices.tex <==
%\appendices

% \section{Supplementary}
\subsection{Reparameterization for Variational Cross-Domain Generation} \label{supp:repara-cross-domain}

In our model, the reparameterization can be written as follows:

\begin{equation}
  \begin{gathered}
    \bm{\ddot{z}}_{st} = \mathcal{G}((\bm \mu_s, \bm \sigma_s), \bm h_t) = \bm \mu_s + \bm \sigma_s \odot (\gamma_1\bm h_t + \gamma_2\bm \epsilon) \\
    \bm {\ddot{z}}_{ts} = \mathcal{G}((\bm \mu_t, \bm \sigma_t), \bm h_s) = \bm \mu_t + \bm \sigma_t \odot (\gamma_1\bm h_s + \gamma_2\bm \epsilon),
    \end{gathered}
    \label{eq:z_addition_appe}
\end{equation}
%where $i$ means the $i$th element. 
In general, consider $\bm h_s \sim p(\mathcal{H}_s) = \mathcal{N}(\bm \mu_{\bm h_s}, \bm \sigma_{\bm h_s})$, and $\bm h_t \sim p(\mathcal{H}_t) = \mathcal{N}(\bm \mu_{\bm h_t}, \bm \sigma_{\bm h_t})$. Adding the standard Gaussian distribution, $\epsilon \sim p(\epsilon) = \mathcal{N}(0, \mathbf{I})$, from Eq.(\ref{eq:z_addition_appe}) we have  $\bm{\ddot{z}}_{st} \sim \mathcal{N}(\bm{\ddot{z}}_{st}; \bm \mu_{st}, \bm \sigma_{st}^2\mathbf{I})$. The $i$-th element of its mean vector can be obtained as
\begin{equation}
\begin{split}
    \mu_{st}^i &= \mathbb{E}\{\mu^i_s + \sigma_s^i(\gamma_1 h_t^i + \gamma_2 \epsilon^i)\}\\
    & = \mu_s^i + \sigma_s^i\gamma_1 E\{h_t\} + \gamma_2 E\{\epsilon^i\} \\
    &= \mu_s^i + \gamma_1 \sigma_s^i \mu_{h_t}^i.
\end{split}
\end{equation}

Ignoring the bias term $\mu_s$, we have the $i$-th element of the variance vector:

\begin{equation}
    \begin{split}
        \mathbf{Var}(\ddot{z}_{st}^i) &= \mathbf{Var}[\sigma_s^i (\gamma_1 h_t^i + \gamma_2 \epsilon^i)]\\
        &=\mathbb{E}\{(\sigma_s^i(\gamma_1 h_t^i + \gamma_2\epsilon^i) - \gamma_1\sigma_s^i\mu_{h_t}^i)^2\} \\
        &= (\sigma_s^i)^2 \mathbb{E}\{[ (\gamma_1 h_t^i + \gamma_2\epsilon^i) - \gamma_1\mu_{h_t}^i]^2\} \\
        &= (\sigma_s^i)^2 \left( \mathbb{E}\{[ (\gamma_1 h_t^i + \gamma_2\epsilon^i)]^2\} - (\gamma_1 \mu_{h_t}^i)^2 \right) \\
        &= (\sigma_s^i)^2 [\gamma_1^2(\sigma_{h_t}^i)^2 + \gamma_2^2].
    \end{split}
\end{equation}
Therefore, the $i$-th element of the standard deviation vector $\bm\sigma_{st}$ is
\begin{equation}
    \sigma_{st}^i = \sigma_s^i \sqrt{\gamma_1^2(\sigma_{h_t}^i)^2 + \gamma_2^2}. 
\end{equation}

There is similar formulation for $\mu_{ts}^i$ and $\sigma_{ts}^i$, as follows:
\begin{equation}
\begin{gathered}
\mu_{ts}^i = \mu_t^i + \gamma_1 \sigma_t^i \mu_{h_s}^i \\
\sigma_{ts}^i = \sigma_t^i \sqrt{\gamma_1^2(\sigma_{h_s}^i)^2 + \gamma_2^2}
\end{gathered}
\end{equation} 



\subsection{Experiments Settings}
\label{supp:experiments_setting}
See Tables 5 -- 6.

\begin{table*}[]
    \centering
    \caption{Experiments Setting for Unsupervised Domain Adaptation}
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
            \hline
            \multirow{2}{*}{Experiments} & \multirow{2}{*}{enc\_style}  & \multirow{2}{*}{Encoder} & \multirow{2}{*}{Decoder} & \multirow{2}{*}{Discriminator} & \multicolumn{2}{|c|}{Encoder Updating} & \multicolumn{2}{|c|}{Decoder Updating} & \multicolumn{2}{|c|}{cls for pixel UDA}   \\
            \cline{6-11}
            &  &    &   &   & LR ($\eta_1$) & optimizer & LR ($\eta_2$) & optimizer &  LR & optimizer  \\
            \hline
            MNIST-MNISTM & fc (128*8)  & \makecell{f32k5s1-\\bn-\\f64k5s2-\\bn-\\f64k5s1-\\bn-\\f128k8s1-\\bn-\\f256k1s2-\\bn-\\f256k1s1}  & \makecell{f128k4s2-\\bn-\\f128k4s1-\\bn-\\f128k4s1-\\bn-\\f64k4s1-\\bn-\\f32k4s2-\\bn-\\f3k1s1}  & fc100-fc2  & \makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 0.0002  & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001  & \makecell{Adam\\($\beta_1$=0.5,\\ $\beta_2$=0.999)}  \\
            \hline
            MNISTM-MNIST & fc (128*8) & - & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.8)} & 0.2 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            MNIST-USPS & fc (128*8) & - & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.8)} & 0.0002 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            USPS-MNIST & fc (128*8) & - & - & -  &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.9)} & 0.001 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.0008 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            FASHION-FASHIONM & fc (128*8) & - & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.8)} & 0.001 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            FASHIONM-FAHSION & fc (128*8) & -  & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.9)} & 0.01 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            Linemod-linemod3D & fc (128*8) & - & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 2e-5 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.0001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)} \\
            \hline
    \end{tabular}}
\end{table*} 

\begin{table*}[]
    \centering
    \caption{Experiments Setting for Unsupervised Image Translation}
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
            \hline
            \multirow{2}{*}{Experiments} & \multirow{2}{*}{enc\_style}  & \multirow{2}{*}{Encoder} & \multirow{2}{*}{Decoder} & \multirow{2}{*}{Discriminator} & \multicolumn{2}{|c|}{Encoder Updating} & \multicolumn{2}{|c|}{Decoder Updating} \\
            \cline{6-9}
            &  &    &   &   & LR ($\eta_1$) & optimizer & LR ($\eta_2$) & optimizer \\
            \hline
            Shoes-edge & fc (128*8)  & \makecell{f32k5s1-\\bn-\\f64k5s2-\\bn-\\f64k5s1-\\bn-\\f128k8s1-\\bn-\\f256k1s2-\\bn-\\f256k1s1} & \makecell{f128k4s2-\\bn-\\f128k4s1-\\bn-\\f128k4s1-\\bn-\\f64k4s1-\\bn-\\f32k4s2-\\bn-\\f3k1s1} & fc100-fc2  & \makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.4)} & 0.002  & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            edge-Shoes & fc (128*8) & - & - & -  &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 0.02 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} \\
            \hline
            CelebA-Sketched CelebA & fc (128*8) & - & - & -  &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 0.2 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            Sketched CelebA-CelebA & fc (128*8) & - & - & -   &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 0.2 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
    \end{tabular}}
\end{table*}

\subsection{More Generation Images}
\label{supp:more_generations}
See Figures 8 -- 18.

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_mnist_mnistm_more_imgs}
   \caption{More Generations in task MNIST(source)-MNISTM(target)}
   \label{fig:mnist_mnistm_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_mnistm_mnist_more_imgs}
   \caption{More Generations in task MNISTM(source) -- MNIST(target)}
   \label{fig:mnistm_mnist_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_mnist_usps_more_imgs}
   \caption{More Generations in task MNIST(source) -- USPS(target)}
   \label{fig:mnist_usps_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_usps_mnist_more_imgs}
   \caption{More Generations in task USPS(source) -- MNIST(target)}
   \label{fig:usps_mnist_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_fashion_fashionm_more_imgs}
   \caption{More Generations in task Fashion(source) -- FashionM(target)}
   \label{fig:fashion_fashionm_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_fashionm_fashion_more_imgs}
   \caption{More Generations in task FashionM(source) -- Fashion(target)}
   \label{fig:fashionm_fashion_more}
\end{figure*}

\begin{figure*}[thpb]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_linemod_more_imgs}
   \caption{More Generations in task Linemod3D(source) -- LinemodReal(target)}
   \label{fig:linemod_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_edge_shoes_more_imgs}
   \caption{More Generations in task Shoes(source) -- edge(target)}
   \label{fig:shoes_edge_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_shoes_edge_more_imgs}
   \caption{More Generations in task edge(source) -- Shoes(target)}
   \label{fig:edge_shoes_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_sketch_face_more_imgs}
   \caption{More Generations in task CelebA(source) -- Sketch(target)}
   \label{fig:face_sketch_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_face_sketch_more_imgs}
   \caption{More Generations in task Sketch(source) -- CelebA(target)}
   \label{fig:sketch_face_more}
\end{figure*}

